Developing and applying heterogeneous phylogenetic models with XRate

Modeling sequence evolution on phylogenetic trees is a useful technique in computational biology. Especially powerful are models which take account of the heterogeneous nature of sequence evolution according to the "grammar" of the encoded gene features. However, beyond a modest level of model complexity, manual coding of models becomes prohibitively labor-intensive. We demonstrate, via a set of case studies, the new built-in model-prototyping capabilities of XRate (macros and Scheme extensions). These features allow rapid implementation of phylogenetic models which would have previously been far more labor-intensive. XRate's new capabilities for lineage-specific models, ancestral sequence reconstruction, and improved annotation output are also discussed. XRate's flexible model-specification capabilities and computational efficiency make it well-suited to developing and prototyping phylogenetic grammar models. XRate is available as part of the DART software package: http://biowiki.org/DART .

==> defs.tex <==
%\usepackage[pdftex]{graphicx}
%\usepackage{graphviz}
\usepackage{verbatim}
% amsmath package, useful for mathematical formulas
\usepackage{amsmath}
% amssymb package, useful for mathematical symbols
\usepackage{amssymb}
%tabularx -for better line wrapping in tables
\usepackage{tabularx}
% graphicx package, useful for including eps and pdf graphics
% include graphics with the command \includegraphics
\usepackage{graphicx}

% cite package, to clean up citations in the main text. Do not remove.
\usepackage{cite}

\usepackage{color} 


% Use doublespacing - comment out for single spacing
\usepackage{setspace} 
\doublespacing


% If-then-else
\usepackage{ifthen}

% algorithms
\usepackage[boxed,noend]{algorithm2e}

% parse trees
%\input{parsetree.sty}

\usepackage{hyperref}

%\bibliographystyle{plain}
%\bibliographystyle{plos2009}

% Remove brackets from numbering in List of References
\makeatletter
\renewcommand{\@biblabel}[1]{\quad#1.}
\makeatother


% Leave date blank
\date{}

\pagestyle{myheadings}

%\newcommand\titlestring{Functional programming for phylogenetic linguistics}
\newcommand\titlestring{Developing and applying heterogeneous phylogenetic models with XRate}
\newcommand\shorttitlestring{Phylogenetic modeling with XRate}

\markboth{\shorttitlestring}{\shorttitlestring}


%% ** EDIT HERE **
%% PLEASE INCLUDE ALL MACROS BELOW

\usepackage{setspace}
\doublespacing


\usepackage{array}


% "Text S1", "Text S2", etc.
\newcommand{\supptext}[1]{Text S#1}

% "Dataset S1", "Dataset S2", etc.
\newcommand{\dataset}[1]{Dataset S#1}

% Labels & references for sections, figures and tables
% Comment out \secref and \seclabel for PLoS -- they don't have numbered section references.
\newcommand{\secref}[1]{Section~\ref{sec.#1}}
\newcommand{\seclabel}[1]{\label{sec.#1}}
\newcommand{\secname}[1]{``#1''}  % PLoS-style section names

% Appendix
\newcommand{\appref}[1]{Appendix~\ref{app.#1}}
\newcommand{\applabel}[1]{\label{app.#1}}

% Table
\newcommand{\tabnum}[1]{\ref{tab.#1}}
\newcommand{\tabref}[1]{Table~\tabnum{#1}}
\newcommand{\tablabel}[1]{\label{tab.#1}}

% Figure
\newcommand{\figref}[1]{Figure~\ref{Figures.#1}}
\newcommand{\figlabel}[1]{\label{Figures.#1}}

% Equation
\newcommand{\eqnref}[1]{Equation~\ref{Equations.#1}}
\newcommand{\eqnlabel}[1]{\label{Equations.#1}}


% need cite, check me, and other notes to self
\newcommand\needcite{{\bf [CITE]}}
\newcommand\checkme{{\bf [CHECK]}}


% Notes by IH
\newcommand\redpen[1]{{\bf \textcolor{red}{#1}} \textcolor{black}{}}
\newcommand\bluepen[1]{{\bf \textcolor{blue}{#1}} \textcolor{black}{}}

\usepackage{lineno}
\linenumbers

